Cross-Modal-Domain Generalization Through Semantically Aligned Discrete Representations

Multimodal learning seeks to integrate information across diverse sensory sources, yet current approaches struggle to balance cross-modal generalizability with modality-specific structure. Continuous (implicit) methods preserve fine-grained priors but render generalization challenging, while discrete (explicit) approaches enforce shared prototypes at the expense of modality specificity. We introduce CoDAAR (Cross-modal Discrete Alignment And Reconstruction), a novel framework that resolves this long-standing trade-off by establishing semantic consensus across modality-specific codebooks through index-level alignment. This design uniquely allows CoDAAR to preserve modality-unique structures while achieving generalizable cross-modal representations within a unified discrete space. CoDAAR combines two complementary mechanisms: Discrete Temporal Alignment (DTA), which enables fine-grained temporal quantization, and Cascading Semantic Alignment (CSA), which promotes progressive cross-modal semantic agreement. Together, they establish a competition-free unified representation space. Trained with self-supervised reconstruction objectives on paired multimodal sequences, CoDAAR demonstrates robust cross-modal and cross-domain generalization. Across Cross-Modal Generalization benchmarks, including event classification, localization, video segmentation, and cross-dataset transfer, CoDAAR achieves state-of-the-art performance, establishing a new paradigm for discrete and generalizable multimodal representation learning.

==> sec/rebuttal.tex <==

\twocolumn[{%
  \centering
  {\Large\bfseries Cross-Modal-Domain Generalization Through Semantically Aligned Discrete Representations\par}
  \vspace{0.4em}
  \centering
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{0.78\textwidth}{!}{%
  \begin{tabular}{l|ccc|ccc|ccc|ccc|c}
    \hline
    \multirow{3}{*}{Method}
      & \multicolumn{6}{c|}{\textbf{VGGSound-AVEL 40K}}
      & \multicolumn{6}{c|}{\textbf{VGGSound-AVEL 90K}}
      & \multirow{3}{*}{Average} \\
    \cline{2-13}
      & \multicolumn{3}{c|}{MSCOCO(V$\leftrightarrow$T)}
      & \multicolumn{3}{c|}{Clotho(A$\leftrightarrow$T)}
      & \multicolumn{3}{c|}{MSCOCO(V$\leftrightarrow$T)}
      & \multicolumn{3}{c|}{Clotho(A$\leftrightarrow$T)}
      & \\
    \cline{2-13}
      & R@1 & R@5 & R@10 & R@1 & R@5 & R@10
      & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & \\
    \hline
    DCID~\cite{xia2023achieving}  & 0.80 & \textbf{5.00} & 8.30 & 2.06 & 9.00 & 16.70 & 0.80 & 4.80 & 8.20 & 2.77 & 11.00 & 20.43 & 7.49 \\
    MICU~\cite{huang2025opensetcrossmodalgeneralization} & \textbf{1.30} & \textbf{5.00} & 8.80 & 2.44 & 10.96 & 18.95 & 0.90 & 4.90 & 9.50 & 3.35 & 10.07 & 17.62 & 7.82 \\
    \textbf{CoDAAR (ours)}                       & 0.80 & 4.40 & \textbf{9.50} & \textbf{3.30} & \textbf{11.57} & \textbf{19.00}
                                                & \textbf{1.30} & \textbf{6.10} & \textbf{10.40} & \textbf{5.64} & \textbf{16.65} & \textbf{24.70} & \textbf{9.45} \\
    \hline
  \end{tabular}
  }
  \captionof{table}{Cross-modal zero-shot retrieval comparison with discrete SOTA methods on MSCOCO (V$\leftrightarrow$T) and Clotho (A$\leftrightarrow$T) datasets.}
  \label{tab:sota_retrieval}
  \vspace{0.4em}
}]

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figs/MICUvCoDAAR.png}
    \caption{Modality dominance comparison of code vectors under AV settings using VGGSound-AVEL 40k pre-training and 400 codewords for \textbf{CoDAAR} and \textbf{MICU}. Red $\rightarrow$ Video dominance, Green $\rightarrow$ Balanced Usage, Blue $\rightarrow$ Audio Dominance}.
    \label{fig:MICUvCodaar}
\end{figure}

\vspace{-1em}

\begin{table}[H]
  \centering
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.12}
  \resizebox{0.65\columnwidth}{!}{%
  \begin{tabular}{l|l|cc|cc}
    \hline
    \multirow{2}{*}{Setting} & \multirow{2}{*}{Cascade}
      & \multicolumn{2}{c|}{\textbf{AVE}}
      & \multicolumn{2}{c}{\textbf{AVVP}} \\
    \cline{3-6}
      &  & V$\!\to$A & A$\!\to$V & V$\!\to$A & A$\!\to$V \\
    \hline
    AVT  & A$\!\rightarrow$T$\!\rightarrow$V & 51.6 & 53.6 & 68.5 & 71.9 \\
         & A$\!\rightarrow$V$\!\rightarrow$T & 51.2 & 52.3 & 70.5 & 73.0 \\
         & V$\!\rightarrow$T$\!\rightarrow$A & 51.4 & 53.8 & 70.0 & 71.4 \\
         & V$\!\rightarrow$A$\!\rightarrow$T & 50.5 & 52.2 & 70.1 & 72.3 \\
    \hline
  \end{tabular}
  }
  \caption{Further cascading order ablation on AVE and AVVP tasks using VGGSound-AVEL 40K pre-training, continued from Table~\ref{tab:cascade_ablation} in the manuscript.}
  \label{tab:cascade_ablation_new}
\end{table}
\vspace{-1em}
\noindent We sincerely thank all reviewers for their constructive feedback and recognition of CoDAAR's contributions.

\noindent\textbf{Reviewer 3tY9:} \textit{(1):}\textit{"Narrow evaluation on audio-video benchmarks; broader retrieval validation needed."} We appreciate this suggestion and have conducted additional zero-shot cross-modal retrieval experiments on MSCOCO (Vision $\leftrightarrow$ Text) and Clotho (Audio $\leftrightarrow$ Text) to validate CoDAAR's broader alignment capabilities (Table~\ref{tab:sota_retrieval}) beyond audio-video benchmarks. CoDAAR achieves the highest overall average score, with robust gains on Clotho A$\leftrightarrow$T retrieval. \textit{(2):} Our design choices are empirically validated through comprehensive ablations (Tables~\ref{tab:ablate_av_40k_ticks},~\ref{tab:ablate_avt_40k_ticks},~\ref{tab:cascade_ablation} in the manuscript, Table~\ref{tab:cascade_ablation_new} here), demonstrating that each component (DTA, CSA, DQA) contributes meaningfully to performance. \textit{(3):} By interpretable, we mean that continuous embeddings rely on opaque contrastive mechanisms, whereas our discrete model explicitly pulls same-index vectors across modalities toward a geometric consensus (CSA), making alignment semantically transparent for downstream decoders. For complexity concerns, we refer to our response to Reviewer PteU. We thank the reviewer for highlighting jargon-heavy passages; we will clarify these sections in the camera-ready version.
% , which lack such explicit interpretability

\noindent\textbf{Reviewer PteU:}
\textit{(1):}\textit{"Complexity vs. practicality concerns":} Contemporary discrete methods (DCID, MICU) employ cross-attention-guided EMA updates and auxiliary losses (CLUB, jigsaw), whereas CoDAAR uses simple mathematical operations (DTA+CSA) for alignment. As shown in Table~\ref{tab:efficiency_singlecol} (Sec.~\ref{sec:efficiency}) in the supplementary materials, this yields faster throughput (14.4 vs. 22.3-25.6 min/epoch), validating that our complementary design reduces rather than adds complexity compared to SOTA discrete methods. \textit{(2):}\textit{"Implicit vs Explicit":} Implicit methods offer strong contrastive alignment but produce unbounded continuous vectors unsuitable for CMG; explicit methods enable downstream modality interchange via shared codebooks but lack robust alignment. CoDAAR bridges this; modality-specific codebooks preserve finite discrete structure (explicit), while DTA and CSA inject cross-modal alignment (implicit).

\noindent\textbf{Reviewer qGcr:} 
\textit{(1):} Together, tables~\ref{tab:cascade_ablation},~\ref{tab:cascade_ablation_new} provide a comprehensive ablation across all six permutations, confirming T$\rightarrow$A$\rightarrow$V as optimal for AVT settings. Dynamic ordering based on entropy/confidence is a valuable suggestion for future work; however, we opted to avoid additional complexity, selecting the order through empirical validation. \textit{(2):} Figure~\ref{fig:MICUvCodaar} compares per-index modality dominance (400 codewords, AV, 40K). MICU shows predominantly video-dominant (red) vectors, validating audio marginalization in shared codebooks; while CoDAAR's concatenated codebook exhibits balanced modality usage (green), demonstrating effective mitigation of representation competition. \textit{(3):} Our hyperparameters follow principled choices: $\lambda_{\text{self}}$, $\lambda_{\text{cross}}$ maintain a 3:1 self-to-cross ratio for stable EMA updates, and $\beta{=}0.25$ follows standard VQ-VAE guidelines. A comprehensive sensitivity analysis is an insightful point and will be included in the camera-ready version due to current page constraints. \textit{(4):} While silence frames may introduce noise during DTA's cross-modal EMA, the subsequent CSA module corrects this by infusing corresponding multimodal semantic information into each modality vector, largely preserving semantic purity.
